Classification of Goods Using Text Descriptions With Sentences Retrieval

The task of assigning and validating internationally accepted commodity code (HS code) to traded goods is one of the critical functions at the customs office. This decision is crucial to importers and exporters, as it determines the tariff rate. However, similar to court decisions made by judges, the task can be non-trivial even for experienced customs officers. The current paper proposes a deep learning model to assist this seemingly challenging HS code classification. Together with Korea Customs Service, we built a decision model based on KoELECTRA that suggests the most likely heading and subheadings (i.e., the first four and six digits) of the HS code. Evaluation on 129,084 past cases shows that the top-3 suggestions made by our model have an accuracy of 95.5% in classifying 265 subheadings. This promising result implies algorithms may reduce the time and effort taken by customs officers substantially by assisting the HS code classification task.

==> 0_guide.tex <==
\section{Message}

마침 교수님께서도 국내 학회 말씀해 주셔서, 인공지능학회 포맷으로 하나 더 만들어봤어요. 데드라인은 10월 12일.\footnote{ \url{http://aiassociation.kr/Conference/ConferenceView.asp?AC=0&CODE=CC20210801&CpPage=122#CONF}} 이 포맷 그대로 LaTeX로 쓰면 되니, 나중에 international conference에 제출할 때 편하겠어요.

영문 2-8장이라고 하니까 한번 쭉 작성해 봐요. Related works나 Introduction 등 작성 가능한 부분들부터 천천히 써 보아요. 우선은 한글이나 영어 중 편한 언어로 작성해고 영문으로 바꿔도 상관 없어요. 여기 일단 제출하는 준비와 함께 84, 90류로 연구 확장해서 1월에 IJCAI나 2월 초 KDD을 목표로 진행해 보죠. 

LaTex 작성 참고 자료로 AAAI에 제출한 domain adaptation 논문과, TKDE에 제출한 active learning 논문 URL 공유해요, 아래 링크에서 compile해서 보면 돼요.

\begin{enumerate}
\item Domain Adaptation 논문: \url{https://www.overleaf.com/read/zbpzfrkpdcnw}
\item Active Learning 논문: \url{https://www.overleaf.com/read/jwbfmjwdrgjj}
\end{enumerate}

이 overleaf 각 파일 하단에 comment 쳐져 있는 내용은 domain adaptation 논문이에요. 양식 참고해요. 

Sep 27: 오늘 교수님하고 나눈 내용 토대로 챕터나 섹션, 하위 섹션, 어떤 그림을 넣을 지 플랜을 짜 보고 Placeholder를 잘 넣어 보세요. 

==> 8_references.tex <==
% \clearpage
\section{References}

Refer to the below example.















\if 0
\paragraph{Code Release.} 
Implementation of \ours{} is included in code supplementaries. We plan to publish an interactive tutorial that contains a series of procedures to compress knowledge, refine data using compressed knowledge, and perform fraud detection.


\paragraph{Data Details.} 
The format of import declarations varied slightly and we only considered the common fields, including numeric variables such as item price, weight, quantity and categorical variables such as HS6 code, country code. The data also contained inspection results indicating whether each declaration was judged fraud or not, and the amount of tax raised after inspection. We 
report the raw variables of import declarations in Table~\ref{Tab:variable_description}. 

\begin{table}[h!]
\centering
\caption{Overview of the transaction-level import data, in which the description of each variable are provided.}
\scalebox{0.75}{
\begin{tabular}{l|l}
\toprule
Variable & Description  \\ \midrule


\textit{Quantity} & The specified number of items\\
\textit{Gross weight} & The physical weight of the items \\
\textit{HS code}   &  Applicable item code based on the harmonised system \\
\textit{Country code}  & Country from which the goods were imported \\
\textit{CIF value} & Transaction value including the insurance and freight costs \\ 
\textit{Total taxes} & Tariffs calculated by initial declaration \\ \midrule
\textit{Illicit ($y$)} & Target binary variable indicating whether the item is fraud \\
\textit{Revenue} & Amount of tax raised after the inspection, used for evaluation \\
\bottomrule 
\end{tabular}}
\label{Tab:variable_description}
\end{table}


\paragraph{Training Details.} 
For every country, the model $f$ is individually pre-trained for 10 epochs and fine-tuned for 30 epochs. The sharpening temperature $\tau$ in Eq~\eqref{eq:SCL_loss} was set as 0.07 by following previous works~\cite{gunel2020supervised}. Smaller temperature for SCL loss benefits training more than
higher ones, but extremely low temperatures are harder to train due to numerical instability. The number of prototypes was set to 500 per class.
We use the final month of each dataset as the test set, and the validation set was chosen as two weeks prior. The model was optimized using Ranger with a weight decay of 0.01~\cite{wright2021ranger21}. The batch size and learning
rate was set as 128 and 0.005 for entire training epochs. All models were run five times, and their average values are reported. 

\paragraph{Baseline Details.} 
Below are the detailed explanation of the baselines used in our experiments.
\begin{itemize}
\item Target Only: Measure the performance of a base fraud detection model $f(\cdot|\mathcal{D}_{t})$ trained on target data. The tree-based embedding model DATE is used~\cite{kim2020date} for $f$. DATE classifies and ranks illegal trade flows that contribute the
most to the overall customs revenue when caught.
\item Vanilla Transfer: Sharing parameters of the fraud detection model $f(\cdot|\mathcal{D}_{s})$ from source country $s$ and directly fine-tune using target dataset $\mathcal{D}_{t}$. 
\item Adaptive Transfer: Adaptive Knowledge Consistency (AKC) technique~\cite{abuduweili2021adaptive} is used to cope with the risk of negative transfer caused by the discrepancy between the source and target countries. It constrains the mean square error between the pre-trained feature extractor outputs and the target feature extractor outputs by adaptively sampling the target dataset $\mathcal{D}_{t}$. We perform a hard filter according to the sample importance by sorting fraud score difference between the source and target pre-trained models. The features with lower 20 \% score difference were selected. 
\end{itemize}



\paragraph{Comprehensive Results.} 
Table~\ref{tab:results_all} shows the comprehensive results, which was simplified in Table~\ref{tab:singlesource} (Single-source scenarios) and Figure~\ref{fig:multisource} (Multi-source scenarios). From Table~\ref{tab:results_all}, we made Table~\ref{tab:singlesource} by picking single-source cases, and we drew Figure~\ref{fig:multisource} by averaging all multi-source \ours{} results grouped by the number of source countries.

Table~\ref{tab:results_label_increase} shows the original results, which was simplified in Figure~\ref{fig:target_size}. The table describes the performance gain by changing the target log size. From Table~\ref{tab:results_all}, we made Figure~\ref{fig:target_size} by averaging \ours{} results grouped by each target country. 

% Table~\ref{tab:results_all} also shows the full result of multi source performance evaluation. The pre-trained model of the source country showing the best performance in the validation set was used. The additional gain in raised tax is most noticeable for using a single source, yet there is a revenue gain with every added source. As the number of source countries increases, performance tends to increase by enriching the information. 


\paragraph{Dependency on Prototype Count.} 
Knowledge of frauds is shared as compressed representations called prototypes. The number of prototypes can determine the resolution of transferred knowledge. For instance, one may assume selective fraud patterns may be shared when we limit the prototype count. We test the sensitivity of the model on prototype count $|\mathcal{C}_s|$ by setting it from 10 to as large as the source data size $|\mathcal{D}_{s}|$. Table~\ref{tab:proto} shows detection performance remains intact by $|\mathcal{C}_s|$, implying that the model is not sensitive to the choice of hyper-parameters as long as the prototypes are used. 

\begin{table}[h!]
\centering
\caption{Sensitivity analysis to the number of prototypes for country N. $|\mathcal{D}_{s}|$ implies that the entire embeddings are transferred instead of the clustered prototypes.}
\small
\scalebox{1}{
\begin{tabular}{c|ccccc}
\toprule
$|\mathcal{C}_s|$ & 0 & 10 & 100        & 1,000   &   $|\mathcal{D}_{s}|$ \\ \midrule
\textsf{M} $\rightarrow$ \textsf{N} & 0.6667  & 0.6714  & 0.6721  & 0.6681 & 0.6709\\
\textsf{C} $\rightarrow$ \textsf{N} & 0.6564 & 0.6656      & 0.6727 & 0.6863 & 0.6711\\
\textsf{T} $\rightarrow$ \textsf{N} & 0.6762 & 0.7379      & 0.7307 & 0.7286 & 0.7314\\
\bottomrule 
\end{tabular}
}
\label{tab:proto}
\end{table}


\input{tables/results_all.tex}
\input{tables/results_label_increase.tex}
\fi

==> algorithms/algo3.tex <==
\begin{algorithm}[h!]
\SetNoFillComment
\begin{flushleft}
 \textbf{Input:} Training set $X_t$, items received $\mathcal{B}_t$, inspection rate $r_t$\\
 \textbf{Output:} A batch of selected items $\mathcal{B}_t^S$ \\
 \SetAlgoLined
 \tcc{Corresponds to the selection part.}
 Train the DATE model using training set $X_t$;\\
 Get the \textsf{Rev@n\%} from validation set;\\
 \eIf{\textsf{Rev@n\%} $\geq \theta$}{
     Perform prediction on $\mathcal{B}_t$, get the predicted annotation $(\textbf{x}_i, \hat{y}_i^{cls}, \hat{y}_i^{rev})$ for each item $\textbf{x}_i \in \mathcal{B}_t$;\\
     Calculate the gradient embedding $g_{x_{i}}$ (Eq. 1);\\
     Obtain the set $\mathcal{B}^S_t$ of $r_t|\mathcal{B}_t|$ items by $k$-means++ initialization;\\
 }{
     Obtain the set $\mathcal{B}^S_t$ of $r_t|\mathcal{B}_t|$ items by random sampling;\\
 }
 \caption{Dummy algorithm template to fill}
 \label{alg:exploration_strategy}
\end{flushleft}
\end{algorithm}

==> tables/datasets.tex <==
\begin{table}[h!]
\centering
% \scriptsize
\small
\caption{Statistics of the datasets}
\label{tab:datastats}
\scalebox{1}{%
\begin{tabular}{ l | r  r  r  r } \toprule
    Country &  \textsf{M} & \textsf{C} & \textsf{N} & \textsf{T}  \\ \midrule
    % Periods & 2013--2016 & 2016--2019 & 2013--2017 & 2015--2019 \\ 
    Duration & 4 years & 4 years & 5 years & 5 years \\ 
    Num. imports & 0.42M & 1.90M & 1.93M & 4.17M  \\ 
    Num. importers & 41K & 9K & 165K & 133K  \\ 
    Num. tariff codes & 1.9K & 5.5K & 6.0K & 13.4K  \\ 
    % GDP per capita & \$300 & \$1,507 & \$2,230 & \$3,317 \\
    GDP per capita & \$300 & \$1,500 & \$2,200 & \$3,300 \\
    % Illicit rate &  1.64\% & 1.71\%   & 4.12\% & 8.16\%  \\ 
    \bottomrule
\end{tabular}
}
\end{table}
